Bias in Internet Measurement Platforms

Network operators and researchers frequently use Internet measurement platforms (IMPs), such as RIPE Atlas, RIPE RIS, or RouteViews for, e.g., monitoring network performance, detecting routing events, topology discovery, or route optimization. To interpret the results of their measurements and avoid pitfalls or wrong generalizations, users must understand a platform's limitations. To this end, this paper studies an important limitation of IMPs, the \textit{bias}, which exists due to the non-uniform deployment of the vantage points. Specifically, we introduce a generic framework to systematically and comprehensively quantify the multi-dimensional (e.g., across location, topology, network types, etc.) biases of IMPs. Using the framework and open datasets, we perform a detailed analysis of biases in IMPs that confirms well-known (to the domain experts) biases and sheds light on less-known or unexplored biases. To facilitate IMP users to obtain awareness of and explore bias in their measurements, as well as further research and analyses (e.g., methods for mitigating bias), we publicly share our code and data, and provide online tools (API, Web app, etc.) that calculate and visualize the bias in measurement setups.

==> sections/acquisition.tex <==
\subsection{Acquisition complexity of ASes}\label{sec:acquisition}

While certain ASes could substantially reduce the overall bias, not all of them might be equally eager to join a project. Some of them might have security, privacy, or communication policies that entirely impede connecting them. In contrast, some ASes (e.g., personal-use ASes) often join projects within hours of first contact. In the following, we study the complexity/cost of adding an AS as a \vp, and how this relates to its impact on the bias score. This acquisition complexity can play a crucial role in practice, and it should not be overlooked when considering vantage point placement.


The complexity for peering with an AS depends on various aspects (operational, legal, etc.). And, to our best knowledge, this dependence has not been publicly reported or studied. Since peering coordinators of route collector projects may manually explore those aspects, we (i) ran a targeted questionnaire among 4 experts involved in 3 route collector projects to record existing domain knowledge, and (ii) build a model to infer the peering complexity for all ASes.

\myitem{Approach overview.} First, we compile a set of labels, based on various datasets, that characterize an AS (with each AS potentially having multiple labels). Then, we asked the peering coordinators to assess---based on their experience---the peering complexity associated with each label. Finally, since each AS is associated with some labels, and each label is mapped to a complexity score, we infer a complexity score for every AS.

\myitem{Characterizing ASes.} ASDB~\cite{ziv2021asdb} combines a multitude of databases and classifiers to associate a set of labels to an AS (e.g., "ISP", "Research and Education", or "Government and Public Administration"). The ASDB dataset characterizes more than 100K ASes with one or more labels (out of 86 potential labels\footnote{ASDB assigns primary and secondary labels. For simplicity, we counted combinations of these two label classes.}). Moreover, we extend the ASDB data with the following labels:

\noindent\textit{Community-support:} ASes that are involved in \imps (by April 1st, 2022), by (i) hosting an active RIPE Atlas probe, or (ii) peering with a RIPE RIS or \rv collector, or (iii) participating in the NLNOG Ring project~\cite{NLNOG2022RING}.

\noindent\textit{Education:} ASNs for which the PeeringDB~\cite{PDB2022WEB} \texttt{info\_type} field in the \texttt{net} record is \texttt{Educational/Research}~\cite{CAIDA2022PDB}, or which are operated by a national research and education network, NRENs (we manually mapped the organization names from Wikipedia~\cite{WIKI2022NRENS} to ASNs using PeeringDB, ipinfo.io~\cite{IPINFO2022ASNMAP}, bgpview.io~\cite{BGPVIEW2022ASNMAP}, bgp.tools~\cite{BGPTOOLS2022ASNMAP}, or their websites).

\noindent\textit{Isolario-peer:} ASes that previously peered with the Isolario route collector project \cite{Isolario2022web} that terminated service on Dec. 31st, 2021. While the MRT data files are no longer publicly available, we extracted the list of peer ASes for each Isolario route collector on June 21st, 2021.

\noindent\textit{Personal-use:} A list of ASes that belong to (mostly) individuals (e.g., as hobby projects, or for testing or research)~\cite{BGPtools2022personal}.

\noindent\textit{Point-of-contact:} We extract from PeeringDB~\cite{CAIDA2022PDB}, all ASNs whose \texttt{role} field in the \texttt{poc} record is either set to \texttt{Maintainance}, \texttt{NOC}, \texttt{Policy}, or \texttt{Technical} as we expect other roles, e.g., \texttt{Abuse}, to not handle peering requests.

\noindent\textit{State-owned:} ASes that are owned (at least partially) by states, based on the list published by Carisimo \etal~\cite{carisimo2021identifying}.






\myitem{Questionnaire \& Complexity Scores} We asked the participants to judge, based on their prior experiences, how much each characteristic/label may influence the ease of peering on a scale from -3 (prevents peering) to +3 (easily peers upon request). Table~\ref{tab:acq:quest_sum} summarizes the answers. While we observe the +3 option twice, we only observed the -3 option once. In general, all participants tended to agree in their answers (with an exception for the "Point-of-contact" label). 



\begin{table}[t]
    \centering
    \caption{Summary of questionnaire answers. The left part corresponds to the ASDB primary labels (and some secondary labels), and the right part to our additional labels.}
    \label{tab:acq:quest_sum}
    \begin{minipage}[t]{0.55\linewidth}
    \begin{tabular}{l r r r}
        \toprule
        \textbf{Label} \phantom{aaaaaa} & \textbf{min} & \textbf{mean} & \textbf{max}  \\
        \midrule
        Community Groups & $\pm 0$ & +1 & +2\\
        ~~~~\& Nonprofits & &&\\
        Computer \& Info. Techn. & $\pm 0$ & +0.25 & +1\\
        Edu. \& Research & $\pm 0$ & +0.25 & +1\\
        Finance \& Insurance & -1 & -0.25 & $\pm 0$\\
        Gov. \& Public Admin. & &&\\
        \quad $\rightarrow$ Military, Security, ... & -3 & -0.75 & $\pm 0$\\
        \quad $\rightarrow$ Other 2nd labels & -1 & -0.25 & $\pm 0$\\
        Services &&&\\
        \quad $\rightarrow$ Law, Business, ... & -1 & -0.25 & $\pm 0$\\
        \quad $\rightarrow$ Other 2nd labels & $\pm 0$ & $\pm 0$ & $\pm 0$\\
        \bottomrule
        %\addlinespace
    \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}{0.4\linewidth}
    \begin{tabular}{l r r r}
        \toprule
        \textbf{Label} \phantom{aaaaaa} & \textbf{min} & \textbf{mean} & \textbf{max}  \\
        \midrule
        Community &$\pm 0$&+0.75& +2\\
        ~~~support &{}&{}&{}\\
        Education & +1 & +1.75 & +2\\
        Isolario-peer & $\pm 0$ & +1.75 & +3\\
        Personal-use &$\pm 0$&+2&+3\\
        Point-of-contact &-2&+0.75&+3\\
        State-owned &-2&-1&$\pm 0$\\
        \bottomrule
        &&&\\
        &&&\\
        &&&\\
        &&&
        %\addlinespace
    \end{tabular}
    \end{minipage}
\end{table}

% \begin{table}[h]
%     \centering
%     \caption{Summary of questionnaire answers. The lower part corresponds to the ASDB primary labels (and some secondary labels), and the upper part to our additional labels.}
%     \begin{small}
%     \begin{tabular}{@{}l r r r@{}}
%         \toprule
%         \textbf{Label ($\rightarrow$ secondary label)} \phantom{aaaaaa} & \textbf{min} & \textbf{mean} & \textbf{max}  \\
%         \midrule
%         Community-support &$\pm 0$&+0.75& +2\\
%         Education & +1 & +1.75 & +2\\
%         Isolario-peer & $\pm 0$ & +1.75 & +3\\
%         Personal-use &$\pm 0$&+2&+3\\
%         Point-of-contact &-2&+0.75&+3\\
%         State-owned &-2&-1&$\pm 0$\\
%         \midrule
%         Community Groups \& Nonprofits & $\pm 0$ & +1 & +2\\
%         Computer and Info. Techn. & $\pm 0$ & +0.25 & +1\\
%         Education and Research & $\pm 0$ & +0.25 & +1\\
%         Finance and Insurance & -1 & -0.25 & $\pm 0$\\
%         Government and Public Admin. & &&\\
%         \quad $\rightarrow$ Military, Security, ... & -3 & -0.75 & $\pm 0$\\
%         \quad $\rightarrow$ Other secondary labels & -1 & -0.25 & $\pm 0$\\
%         Services &&&\\
%         \quad $\rightarrow$ Law, Business, and Consulting & -1 & -0.25 & $\pm 0$\\
%         \quad $\rightarrow$ Other secondary labels & $\pm 0$ & $\pm 0$ & $\pm 0$\\
%         \bottomrule
%         %\addlinespace
%     \end{tabular}
%     \end{small}
%     \label{tab:acq:quest_sum}
% \end{table}

% In the second part, we provided two AS characterisations (e.g., Tier 1 transit provider vs content provider) and asked which one would be harder to acquire as a peer. While the answers from this part mostly confirmed the answers from the previous part, it also highlighted that AS are perceived as harder to peer with solely on the country that they are operated in. \todo{shall we add the ODIN rankings?}

For each label, we take the mean value across all questionnaire answers. For each AS, we merge the different labels as follows: if there is a -3 or +3 label, we set the complexity score to -3 or +3 (preferring -3 over +3), respectively, otherwise we take the mean across all labels; this approach ensures that our final values always comply with the strong indications provided by the experts.\pamout{\footnote{We tested different merging approaches and/or using the min/max instead of the average values. Detailed results can be found in Appendix~\ref{appendix:questionnaire-merging}}} Finally, we divide this score by 3 to normalize it.

\myitem{Complexity scores for current and future ASes.}
Figure~\ref{fig:acq:platf} (black curve, "All") shows the distribution of acquisition complexity scores across all ASes: approximately 80\perc of ASes are equally hard to peer with, while the remaining 20\perc split almost equally between ASes that are substantially harder/easier to peer with. Comparing with the distributions of ASNs that are part of \imps, we can see that
all platforms are biased towards easier-to-connect ASes; this trend is stronger for RIPE Atlas as only \textasciitilde 17\perc of probe hosting ASes have equal or lower complexity scores than the median AS (i.e., \textasciitilde 0.1).

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.4\linewidth]{figures/acquisition/weights_per_platform.pdf}\label{fig:acq:platf}}
    \hspace{0.1\linewidth}
    \subfigure[]{\includegraphics[width=0.4\linewidth]{figures/acquisition/biasdiff_vs_weights.pdf}\label{fig:acq:bias}}
    \caption{(a) Distribution of acquisition complexity across different platforms. (b) Bias difference vs. complexity scores as heatmap (outliers denoted as markers).}
\end{figure}


\textit{Does this mean that decreasing the bias can only be achieved by convincing hard-to-connect ASes?} Figure \ref{fig:acq:bias} shows a heatmap that compares these two dimensions for the RIPE RIS platform. We can observe that there is no strong correlation, i.e., there is no pattern indicating that networks that could decrease bias are harder to connect to. Moreover, there are several ASNs that are ideal candidates to extend RIPE RIS (top left part of the heatmap), since they could significantly decrease bias and are easy to connect. For example, AS132139 %(VECLOUD LIMITED)
---a cloud on-ramp provider\footnote{An AS that mainly provides transit to all major cloud providers / hypergiants.} with three upstreams that mainly operates in Hong Kong, is registered under APNIC, and announces few IPv4 and IPv6 prefixes---would be a great choice for extending RIPE RIS as it has labels that indicate a low peering complexity (0.66) and also reduces the bias drastically (-0.59\%). 

\myitem{Summary of main takeaways:} \one Adding extra a few hundreds \vps to \imps can decrease their bias by 50\%; \two While \textasciitilde10\perc of ASes are easy to acquire as new \vps, another \textasciitilde10\perc of ASes need substantial effort to be connected; \three There is a very clear set of extension candidates that can easily be connected and substantially reduces bias.%; and \four Alternative goals (e.g., reducing the number of hops to each origin) can be achieved while reducing the overall bias of an \imp. 


%\todo{Discuss feed acquisition procedure: The infrastructure deployment processes are the root cause for the observed bias in the Internet measurement platforms (e.g., RIPE NCC has largest coverage in its service region, and most route collectors are located in IXPs).}



% Yet, it is very rare that researchers and operators pick data from either RIS or \rv instead of both. While our methodology can be used for arbitrary sets of ASNs (i.e., using it to optimize extension candidates for the union of two platforms requires no changes), it is unclear how realistic multi-platform goals can be realized. Different platforms---especially when also considering other projects such as PCH, (previously) Isolario, or bgp.tools (which also provides BGP data on explicit request)---might have different requirements and incentives for peer acquisitions or simply lack motivation or staffing to enter multi-platform coordination. 

==> sections/acquisition__backup_13May.tex <==
\subsection{Acquisition Complexity}
\begin{figure*}[h!tb]
        \minipage[t]{0.32\textwidth}
          \includegraphics[width=\linewidth]{figures/acquisition/weights.pdf}
          \caption{Distribution of Acquisition complexity using different aggregation approaches.}\label{fig:acq:weights}
        \endminipage
    \hfill
        \minipage[t]{0.32\textwidth}
          \includegraphics[width=\linewidth]{figures/acquisition/weights_per_platform.pdf}
          \caption{Distribution of Acquisition complexity across different platforms.}\label{fig:acq:platf}
        \endminipage
    \hfill
        \minipage[t]{0.32\textwidth}
          \includegraphics[width=\linewidth]{figures/acquisition/biasdiff_vs_weights.pdf}
          \caption{Bias difference vs acquisition complexity per asn as heatmap (with added outliers).}\label{fig:acq:bias}
        \endminipage
\end{figure*}
While certain peers may substantially reduce the overall bias in a platform, not all of them might be equally eager to join a project. Some of them might have security, privacy, or communication policies that entirely impede connecting them. In contrast, some ASNs (e.g., toy or personal-use ASNs) often join projects within hours of first contact.

The position of an AS along this complexity dimension depends on various aspects such as time to first contact, operational willingness to peer, or legal peering requirements. While dedicated peering coordinators may manually explore those aspects for certain ASes, scaling this approach to our needs is infeasible. Hence, we relied on a two-stage approach: In the first stage, we ran a questionnaire among the peering co-ordinators as well as current and former maintainers of RIPE RIS, \rv, and Isolario\footnote{We also contacted the maintainers of the Packet Clearing House project~\cite{PCH2022WEB} but, after a month, did not receive an answer.} to assess how certain characteristics of an AS facilitate or complicate its acquisition as a peer. In the second stage, we labeled each AS with a set of such characteristics using various data sets and then collapsed the labels for each ASN to a single `ease of acquisition` value. While the first step heavily informed the second step (e.g., it dictated for which labels we had to acquire data sets), we'll first discuss the labeling process and then the questionnaire's outcomes as well as the resulting per-AS values. 

\subsubsection{Characterising ASes}
To bootstrap the labeling process, we rely on ASDB~\cite{ziv2021asdb}. ASDB combines a multitude of databases and machine learning classifiers to associate a set of characterization labels (e.g., "ISP", "Research and Education", or "Government and Public Administration") to each AS. The latest version (from 25th Nov. 2022) describes more than 100K ASes using between 1 and 28 (out of 86 potential) labels\footnote{ASDB actually assigns primary and secondary labels. For simplicity, we counted combinations of these two label classes}. 

We extend ASDB's label set with the following labels: \\
\textbf{Community-support:} ASes that actively provide data or measurement opportunities to platforms frequently used by the community. We obtained this list by joining four different lists (all gathered on April 1st, 2022): \one ASes that host an RIPE Atlas probe for which the status is active, \two ASes that peer with an RIPE RIS collector, \three ASes that peer with an \rv collector, and \four ASes that participate in the NLNOG Ring project~\cite{NLNOG2022RING}.\\
\textbf{Education:} ASNs for which the PeeringDB \texttt{info\_type} field in the \texttt{net} record specified \texttt{Educational/Research} or which are operated by a national research and education networks (NRENs). For the first list, we used a snapshot of PeeringDB~\cite{PDB2022WEB} from April 1st, 2022 that was hosted by CAIDA~\cite{CAIDA2022PDB}. For the second list, we obtained a set of organisation names from Wikipedia~\cite{WIKI2022NRENS} and then manually\footnote{Please note that an automated approach against, e.g., IANA/RIR delegation information seemed infeasible due to differences in naming schemes and (mostly subtle, yet hard to generically program) deviations from Wikipedia's exact spelling.} mapped these organisation names to ASNs using PeeringDB, ipinfo.io~\cite{IPINFO2022ASNMAP}, bgpview.io~\cite{BGPVIEW2022ASNMAP}, bgp.tools~\cite{BGPTOOLS2022ASNMAP}, or the respective organization's website.\\
\textbf{Isolario-peer:} ASes that previously peered with the Isolario Route Collector project~\cite{Isolario2022web} that terminated service on December 31st, 2021. While the MRT data files are no longer publicly available, we extracted the list of peer ASes for each Isolario route collector on June 21st, 2021 as part of an unrelated project.\\
\textbf{Personal-use:} ASes that belong to (mostly) individuals that maintain them as hobby projects or for testing and researching activities. The list of such ASes hosted at bgp.tools~\cite{BGPtools2022personal} was gathered and updated over years via discussions with the operator community.\\
\textbf{Point-of-contact:} Using the previously mentioned PeeringDB snapshot, we extract all ASNs for which the \texttt{role} field in the \texttt{poc} record is either set to \texttt{Maintainance}, \texttt{NOC}, \texttt{Policy}, or \texttt{Technical} as we expect other roles, e.g., \texttt{Abuse} to not handle peering requests; please note that organisations may enter multiple points of contact with different roles.\\
\textbf{State-owned:} ASes that are owned (at least partially) by states, based on the list published by Carisimo \etal~\cite{carisimo2021identifying}.\\





\begin{table}[t!hb]
    \centering
    \begin{tabular}{@{}l r r r@{}}
        \toprule
        \textbf{Label ($\rightarrow$ secondary label)} \phantom{aaaaaa} & \textbf{min} & \textbf{mean} & \textbf{max}  \\
        \midrule
        Community-support &$\pm 0$&+0.75& +2\\
        Education & +1 & +1.75 & +2\\
        Isolario-peer & $\pm 0$ & +1.75 & +3\\
        Personal-use &$\pm 0$&+2&+3\\
        Point-of-contact &-2&+0.75&+3\\
        State-owned &-2&-1&$\pm 0$\\
        \midrule
        Community Groups \& Nonprofits & $\pm 0$ & +1 & +2\\
        Computer and Info. Techn. & $\pm 0$ & +0.25 & +1\\
        Education and Research & $\pm 0$ & +0.25 & +1\\
        Finance and Insurance & -1 & -0.25 & $\pm 0$\\
        Government and Public Admin. & &&\\
        \quad $\rightarrow$ Military, Security, ... & -3 & -0.75 & $\pm 0$\\
        \quad $\rightarrow$ Other secondary labels & -1 & -0.25 & $\pm 0$\\
        Services &&&\\
        \quad $\rightarrow$ Law, Business, and Consulting & -1 & -0.25 & $\pm 0$\\
        \quad $\rightarrow$ Other secondary labels & $\pm 0$ & $\pm 0$ & $\pm 0$\\
        \bottomrule
        %\addlinespace
    \end{tabular}
    \caption{Summary of questionnaire answers. \textmd{While the lower half shows ASDB's primary labels (and some secondary labels), the upper half shows our additional labels.}}
    \label{tab:acq:quest_sum}
\end{table}


\subsubsection{Questionnaire results}
Now that we have introduced our labeling process, we can take a closer look at our questionnaire and its outcomes. The questionnaire was mainly composed of two parts. In the first part, we asked the participants to judge, based on their prior experiences, how much each characteristic may influence the ease of acquisition on an Integer scale from -3 (prevents peering) to +3 (guarantees peering upon request). Table~\ref{tab:acq:quest_sum} summarizes the four answers that we got. While we observe that +3 option twice, we not once observed the -3 option. This may indicate that all ASes may be acquired as peers given the right constraints, incentives, and time. Apart from these extremes, all answers showed usually the same tendencies except for the "Point-of-contact" characteristic; here, one participant evaluated the characteristic as substantially hindering (-2) while all others evaluated it as beneficial (+1, +1, and +2). We were not able to figure out the reason for this specific judgement as the questionnaire was entirely anonymized and the participant did not include further information in the available text fields. 

In the second part, we provided two AS characterisations (e.g., Tier 1 transit provider vs content provider) and asked which one would be harder to acquire as a peer. While the answers from this part mostly confirmed the answers from the previous part, it also highlighted that AS are perceived as harder to peer with solely on the country that they are operated in. \todo{shall we add the ODIN rankings?}

\subsubsection{Collapsing labels.} By the end of our labeling process, most ASes have multiple labels. Given that we extracted the min, mean, and max answers for each label from the questionnaire and could take the min, max, or some merged value across all labels that are assigned to an ASN, we end up with nine different variations of how we could collapse the label set of an AS to a single ease-of-acquisition value. Please note that, instead of simply averaging them, we decided to merge values as follows: \one if there is -3 label, set the final value to -3, \two if there is a +3 label, set the final value to +3, and \three take the mean across all labels; this approach ensures that our final value always complies with ``guaranteed not`` and ``guaranteed.`` Before analysing the results and deciding for a collapsing policy, we divided all values by 3 to normalize them. 

Figure~\ref{fig:acq:weights} shows the ECDF of ease-of-acquisition values across all ASes for five of the before-mentioned nine collapsing approaches (the remaining four curves lie between the min/min and max/max curve and are hidden to preserve the clarity of the plot).  We observe that all curves show similar tendencies: Approximately 80\perc of ASes are equally hard to peer with, while the remaining 20\perc split almost equally between ASes that are substantially harder/easier to peer with. As the insides from the min/min and max/max curve are properly reflected by it, we decide to continue with the avg/merge collapsing approach for the remainder of this paper. 


\subsubsection{State of current platforms.} Before looking into extending platforms, we first want to understand the current participant base of each platform. Figure~\ref{fig:acq:platf} shows an ECDF over the ease-of-acquisition values across all participants of a given platform. The "all" curve resembles the distribution across all ASes (i.e., it is the same curve from the previous figure). While we observe that all platforms are biased towards easier-to-connect ASes, we observe that this trend is exceptionally strong for RIPE Atlas as only \textasciitilde 17\perc of probe hosting ASes have equal or lower ease-of-acquisition than the median AS (i.e., \textasciitilde 0.1). 

\subsubsection{Picking new participants.} After this brief look at the current participant base of each platform, we now want to see whether there is a correlation between an AS' potential to reduce a platform's bias and its ease of acquisition. Figure \ref{fig:acq:bias} shows a heatmap (as well as outliers for the  cells in which the color is barely visible) that compares the these two dimensions when extending the RIPE RIS platform. \todo{You can find figures for the other platforms in the appendix.} While we observe no strict correlation, we find a set of strong connection candidates, e.g., AS132139 (VECLOUD LIMITED)---a cloud on-ramp provider\footnote{i.e., an AS that mainly provides transit to all major cloud providers (also called hypergiants).} with three upstreams that mainly operates in Hong Kong, is registered under APNIC, and announces few IPv4 and IPv6 prefixes---would be a great choice for extending RIS as it is easy to connect (0.66) and also reduces the bias drastically (-0.59). 

In general, all ASes in the top-left corner seem like ideal candidates to extend RIPE RIS. Yet, it is very rare that researchers and operators pick data from either RIS or \rv instead of both. While our methodology can be used for arbitrary sets of ASNs (i.e., using it to optimize extension candidates for the union of two platforms requires no changes), it is unclear how realistic multi-platform goals can be realized. Different platforms---especially when also considering other projects such as PCH, (previously) Isolario, or bgp.tools (which also provides BGP data on explicit request)---might have different requirements and incentives for peer acquisitions or simply lack motivation or staffing to enter multi-platform coordination. 

\pavlos{TBD if we include this. Discussion about how to extend infrastructure; e.g., (i) cost of adding infra (vs bias), (ii) other gains such as visibility/proximity/completenss (vs bias) - decreasing bias is not the only objective. And (iii) propose algorithm for decreasing bias.}


==> sections/ethics.tex <==
We carefully designed this study to protect user privacy and conduct ethical research. 


\subsection{Questionnaires} 

Throughout this study, we circulated two \textit{anonymous} questionnaires via Google Forms~\cite{Google2022Forms}. We do not collect personal data in any of the questionnaires.

In both questionnaires, we follow the basic principles of ethical research ("Respect for Persons": voluntary, informed participation, etc.;  "Beneficence": no harm, returning benefits by sharing the findings/tools of our research, etc.; "Justice": publicly accessible data, code, etc.), as well as the guidelines for collecting anonymous (no personal) data through online surveys, namely, by insuring informed consent, information, comprehension, voluntariness, returning benefits, minization of risks, and a fair selection of participants.

Specifically, the first questionnaire was circulated publicly (mainly though network operators mailing lists and social media) and displayed the following text on its landing page:

"This survey is part of a research effort by the \dbsub{AI4NetMon} project (\dbsub{https://sermpezis.github.io/ai4netmon/}) to study the Internet monitoring / measurement practices, common use cases, and potential biases. We expect the findings of this survey to contribute towards developing methods, tools, and recommendations for improving the Internet monitoring infrastructure and practices.

The questionnaire should be filled out by professionals whose work relates to Internet operations (e.g., network operators or researchers). It should take no longer than 10 minutes to answer. 

Research records will be kept confidential to the extent allowed by law. All collected data will be anonymous and published in a manner that would not allow identification of the participants' personal identity. A summary of the aggregate results will be published as a part of an article and/or conference paper. 

If you agree to participate in this study, please answer the questions of this survey (do NOT include in your answers information that may help to identify you or your organization). Participation in this study is voluntary. You have the right to not participate at all or to leave the study at any time without penalty or loss of benefits to which you are entitled. If you have any feedback on the survey, or would like to be notified when we publish a summary of results, or you want additional information, please write us at \dbsub{sermpezis@csd.auth.gr}.

Contact information: <first author's contact information>."\\

The participants had to explicitly click on "continue" to leave this landing page and actually enter the questionnaire. 


The second questionnaire was forwarded privately to few selected individuals with whom we already had prior interactions. When forwarding, we similarly included information about the research we conduct, the motivation behind the questionnaire, and how we would incorporate the resulting information.

The participants remained fully anonymous. We did not request any information that could identify a single individual. To minimize the risk of identifying individuals by cross-referencing other public data sources~\cite{narayanan2008robust}, we will neither publish the raw answers nor preprocessed versions of individual answers in any form. Further, we believe that the questionnaire descriptions and answer summaries that we provide throughout this paper do not allow for the re-identification of individual participants. 




\subsection{AS characteristics} 


While our study only assigns labels to AS numbers (acquisition complexity; see \secref{sec:acquisition}), the names associated with these AS numbers sometimes identify single individuals, e.g., when the AS is a hobby/toy AS of that individual. Hence, we only share the final complexity score per AS but none of the intermediate data formats that associate ASNs with sets of characteristics. Please note that these complexity scores were explicitly calculated to estimate the chances that an AS peers with route collectors (i.e., a very special, niche class of networks) and can not reflect an AS' general peering complexity.  

Also, we explicitly mention in the text, that these complexity scores are "inferences" and may not be true for each and every AS sharing these labels.

Moreover, the bias scores we calculate do not correspond to and/or characterize individual networks, but rather they are defined in the context of sets of networks. A bias score characterizes a set of networks and indicate how representative this set is wrt. to the entire population of ASes. Having a high bias score only means that this set is not representative of the entire population. A network can belong to a set with high bias score, and at the same time to a set with a low bias score. 


\subsection{CDN measurements} 

For our use case analysis (\secref{sec:cdn-use-case}), we collaborated with a large production CDN. The CDN follows various strict policies to retrieve anonymized performance statistics as a part of their routine network analysis. The individual data points presented in this paper were entirely produced on servers located at the CDN's premise. The visualization of the data points was produced outside the CDN's premise, however, they correspond only to aggregate information, and do not carry any per-individual or per-network information or can be used to infer this information.

==> sections/ethics_short.tex <==
We carefully designed this study to protect user privacy and ethical research. 


\myitem{Questionnaires.} Throughout this study, we circulated two \textit{anonymous} questionnaires. We do not collect any personal data, and we follow the basic principles of ethical research (Respect for Persons, Beneficence, Justice, etc.), and the guidelines for collecting anonymous data through online surveys (informed consent, comprehension, voluntariness, returning benefits, minimization of risks, etc.). To minimize the risk of identifying individuals, we will neither publish the raw or preprocessed versions of individual answers. 




\myitem{AS characteristics.} (i) The complexity score we inferred for each AS indicates the chances that an AS peers with route collectors, and (ii) the bias score is calculated for a set of networks and indicates how representative this set is wrt. the entire population of ASes; none score characterizes in any other way an AS.


\myitem{CDN measurements.} In our use case (\secref{sec:cdn-use-case}), we collaborated with a large CDN with strict policies to retrieve anonymized performance statistics. The individual data points presented in this paper were entirely produced on servers at the CDN's premise, and do not carry any per-individual or per-network information.

==> sections/extension.tex <==
The bias of \imps can be decreased by adding new participants from under-represented dimensions. In this section, we take a closer look at the effectiveness (\secref{sec:extra-infra-selection}) and complexity (\secref{sec:acquisition}) of adding vantage points. %We limit our analysis to the RIPE RIS and \rv platforms, where the existence of bias is more significant (see Section~\ref{sec:bias-results}) and have much less monitors than RIPE Atlas.

\subsection{Selecting new vantage points}\label{sec:extra-infra-selection}
As our framework can calculate bias for arbitrary sets of \vps, we can calculate the difference in bias that a given \vp $v$ would introduce by adding it to the existing set of \vps of a platform $\mathvp$, i.e., 
\begin{equation}\label{eq:bias-plus-one}
    B(\mathvp\cup\{v\}) \leftarrow calculate\_bias(\mathcal{N}, \mathvp\cup\{v\})
\end{equation}
This problem shares the same hardness and complexity properties as the subsampling problem we discussed in~\secref{sec:subsampling-algorithms}. Hence, we again may rely on either a sorting or a greedy strategy: The algorithm sorts \vps based on how they affect bias (Eq.~\ref{eq:bias-plus-one}) and either \one selects the $k$ \vps that decrease the bias score the most  (sorting algorithm) or \two greedily chooses the $v$ that minimizes the \imp bias (i.e., $v \leftarrow \arg\min B(\mathvp\cup\{v\})$) in each iteration and adds it to the set of all \vps $\mathvp$.
Despite its similarity to the subsampling variant, this greedy algorithm has a much higher complexity of $O\left(|\mathcal{N}|\cdot |\mathvp|^{2}\right)$. Since the algorithm has to investigate $\mathcal{N}\backslash\mathvp$ vantage points in each iteration and $\mathcal{N}$ is multiple orders of magnitude larger than $\mathvp$, the algorithm effectively runs in $\gg O\left(|\mathvp|^{3}\right)$.

\myitem{Extending RIPE RIS and \rv.} For RIPE RIS and \rv, we calculate the bias difference for every\footnote{In this analysis we omit stub ASes, i.e., edge networks having only one neighbor AS and connecting to the Internet through this single upstream provider.} AS not in \imps (using Eq.~\ref{eq:bias-plus-one}), and present the distribution of these differences in Fig.~\ref{fig:extra-infra-cdf}. While few ASes would further increase the bias (i.e., values larger than 0.0), the vast majority of ASes would decrease the bias (i.e., negative values); this shows that there are many good options for extending the route collector projects. We further observe that certain ASes are especially beneficial as they would decrease the bias score by more than 2\% for \rv or almost 1\% for RIPE RIS.

Yet, substantially decreasing the bias of a platform requires greater efforts than connecting a single AS.
Using the sorting algorithm, Fig.~\ref{fig:extra-infra-bias-vs-monitors} shows how the bias for these platforms reduces with increasing amounts of new ASes. The bias in both RIPE RIS and \rv can decrease to a value of 0.05 with a few hundreds of extra \vps (which is close to the minimum value achieved by subsampling; see Fig.~\ref{fig:bias-vs-sample-size-greedy-all}), while \rv would need less extra \vps compared to RIPE RIS to reach a certain bias score value.


\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.4\linewidth]{figures/fig_cdf_bias_diff_rel__no_stubs.png}\label{fig:extra-infra-cdf}}
    \hspace{0.1\linewidth}
    \subfigure[]{\includegraphics[width=0.4\linewidth]{figures/fig_cdf_bias_vs_nb_extra_monitors.png}\label{fig:extra-infra-bias-vs-monitors}}
    \caption{(a) Distribution (over all ASNs) of the relative difference in the bias score by adding an extra ASN in the measurement platforms, i.e., $100\% \cdot \frac{B(\mathvp\cup\{m\})}{B(\mathvp)}$. (b) Average bias score (y-axis) of the measurement platforms by adding an extra number of monitors (x-axis) selected by a sorting algorithm.}
    \label{fig:extra-infra}
\end{figure}

% \subsection{Bias vs Monitoring Efficiency}
% \pavlos{The above algorithm does not take into account other gains by adding new infrastructure. Do an analysis of other added values (see below).}
% \pavlos{The following is a preliminary version (almost placeholder)}
% Adding a monitor improves our visibility of the Internet. E.g., a route collector peer can reveal new AS links. We study the trade-off between bias and different `improvement scores'. For example, we can consider the following improvement dimensions
% \begin{itemize}
%     \item number of new AS links revealed
%     \item visibility to unseen (or poorly seen) prefixes
%     \item closeness to edge networks (in terms of AS hops) or IXPs
%     \item other??
% \end{itemize}

% The methodology can be: We assume a that a subset of monitors $\hat{\mathvp}\subset\mathvp$ are not part of the infrastructure. We calculate the difference in bias with and without them (i.e., the bias of the sets $\mathvp$ and $\mathvp\backslash \hat{\mathvp}$, respectively). We calculate the improvement score by $\hat{\mathvp}$. We present results, such as correlations between bias and improvement, or scatter plots, etc. E.g., Figure~\ref{fig:bias-vs-improvement} (note: the current version of the figure is for networks that are not currently part of the infrastructure).

% \myitem{Research questions} (to be answered by the results)
% \begin{itemize}
%     \item Can we have both good improvement and low bias? \item If yes, what are the characteristics of networks that achieve this?
% \end{itemize}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{./figures/Fig_scatter_bias_vs_improvement.png}
%     \caption{Bias vs improvement}
%     \label{fig:bias-vs-improvement}
% \end{figure}




% \subsection{Cost of adding new infrastructure}
% \pavlos{The above algorithm does not take into account the cost. Now take it into account. How? Survey results? Show some results for cost effective selection (e.g., select only from the set of low cost)}


==> sections/subsampling.tex <==

The bias of the \imps is due to the fact that some types of networks are under-represented and others over-represented (e.g., networks in Asia and Europe, respectively, for RIPE Atlas; see Fig.~\ref{fig:example-distribution-location}). To decrease the bias, we need to have a balanced representation of all network types.
%
To this end, we can either (i) deploy new \vps to the under-represented network types or (ii) use only a subset of the existing monitors whose types are over-represented. In this section, we study the latter option, which is immediately applicable and does not involve any extra costs. We study aspects of extending the \imps in~\secref{sec:extra-infrastructure}.

% There are two ways to achieve this: (i) The first is by deploying new monitors to the under-represented network types. This would also increase our coverage of the Internet routing system and would offer extra options for conducting measurements. However, this involves some significant costs for the deployment and operation of the infrastructure (e.g., hardware, data management, operational costs).
% (ii) The second way, is by considering only a subset of the networks in the infrastructure whose types are over-represented, i.e., by using a (carefully selected) sub-sample of the infrastructure.


\subsection{Subsampling: problem and algorithms}\label{sec:subsampling-algorithms}

We consider the problem of selecting a subset of \vps in the \imps (subsampling), whose bias is lower than the bias of the entire set of \vps; or, more formally: 
\begin{equation}
    \textstyle \min_{\mathcal{S}\subseteq\mathvp} B(\mathcal{S})
\end{equation}
where $\mathcal{S}$ is a subset of the \vps of a \imp, $\mathcal{S}\subset\mathvp$, and $B(\mathcal{S})$ is its bias score, which we want to be less than the bias of the entire set of \vps in the \imp ($B(\mathcal{S}) < B(\mathvp)$). Optionally, we may impose constraints, e.g., to require a given size of the subset ($|\mathcal{S}| 
\leq k$). 


\myitem{Problem complexity.} The above problem is combinatorial, and relates to the best subset problem with cardinality constraints, which is NP-hard~\cite{bertsimas2016best}. Moreover, it is straightforward to show (through counter-examples) that it lacks the properties of \textit{monotonicity} and \textit{submodularity}, which would allow to design approximation algorithms with performance guarantees% by constructing the set $S$ through greedy selection (one by one) of monitors
~\cite{krause2012submodular}. Informally, the complexity of the problem is due to the fact that adding a \vp in a set could either decrease or increase bias (no monotonicity). And, since the bias score is calculated over distributions of characteristics for the entire set of selected \vps (see Equation~\ref{eq:bias-metric-kl}), having two \vps can be equally, less, or more than the sum of effects of adding each \vp individually (no submodularity). 


\myitem{Greedy algorithm.} We design a heuristic algorithm to select a subset of \vps with low bias (Algorithm~\ref{alg:subsampling-greedy}). The algorithm starts by considering the entire set of \vps in the \imp $\mathvp$. Then, for every \vp $v\in\mathvp$, it calculates the resulting bias score if we remove this \vp from the \imp, i.e., the bias score of the set\footnote{$A\backslash B$ denotes all elements in a set A, except for those that belong also to a set B.} $\mathvp\backslash\{v\}$ (see lines 2--4). And, it removes from the set $\mathvp$ the \vp $v$ that would decrease the most the bias score, i.e.,  $\arg\min_{v} B(\mathvp\backslash\{v\})$ (lines 5--6). It repeats the above process for the updated set $\mathvp$ by removing one \vp at each iteration, until the remaining set is of the desired size $k$. 

\pamout{\textit{Remark:} If the subset size $k$ is not crucial, we can include a termination condition to end the loop when there are no other \vps whose removal decreases the bias (i.e., when $Bias(\mathvp\backslash\{v\}) \geq Bias(\mathvp), ~\forall v\in\mathvp$).} 

The complexity of the algorithm is $O\left((|\mathvp|-k)\cdot |\mathvp|^{2}\right)$, or $\approx O\left( |\mathvp|^{3}\right)$ for small $k$, since the loop in lines 1--7 is executed $|\mathvp|-k$ times, and the loop in lines 2--4 is executed $|\mathvp|-i$ times at the $i^{th}$ iteration (i.e., complexity $O(|\mathvp|)$, and the calculation of bias in line 3 requires the calculation of the distribution $P$ (probabilities $p_{i}$ in Equation~\ref{eq:bias-metric-kl}) which is of complexity $O(|\mathvp|)$.

\begin{figure}
\centering
\begin{minipage}[t]{0.45\linewidth}
\centering
\captionof{algorithm}{\textbf{Greedy}}
\label{alg:subsampling-greedy}
\begin{algorithmic}[1]
    \Statex {Input: $\mathcal{N}$ (population), $\mathvp$ (vantage points), $k$ (sample size)} 
    \While{$|\mathvp|>k$}
        \For{$v\in\mathvp$}
            \State $B_{v} \leftarrow calc\_bias(\mathcal{N}, \mathvp\backslash\{v\})$
        \EndFor
        \State $v\leftarrow \arg\min B$
        \State $\mathvp\leftarrow \mathvp\backslash\{v\}$
    \EndWhile
    \State Return $\mathvp$
\end{algorithmic}
\end{minipage}
\hspace{0.05\linewidth}
\begin{minipage}[t]{0.45\linewidth}
\centering
    \captionof{algorithm}{\textbf{Sorting}}
    \label{alg:sorting}
    \begin{algorithmic}[1]
    \Statex {Input: $\mathcal{N}$ (population), $\mathvp$ (vantage points), $k$ (sample size)} 
    \For{$v\in\mathvp$}
        \State $B_{v} \leftarrow calc\_bias(\mathcal{N}, \mathvp\backslash\{v\})$
    \EndFor
    \While{$|\mathvp|>k$}
        \State $v\leftarrow \arg\min B$
        \State $\mathvp\leftarrow \mathvp\backslash\{v\}$
    \EndWhile
    \State Return $\mathvp$
    \end{algorithmic}
\end{minipage}
\captionof{figure}{Subsampling algorithms}
\end{figure}




% \begin{algorithm}
% \begin{small}
% \begin{algorithmic}[1]
% \caption{Subsampling - Greedy}\label{alg:subsampling-greedy}
% \Statex {Input: $\mathcal{N}$ (population), $\mathvp$ (vantage points), $k$ (sample size)} 
% \While{$|\mathvp|>k$}
%     \For{$v\in\mathvp$}
%         \State $B_{v} \leftarrow calculate\_bias(\mathcal{N}, \mathvp\backslash\{v\})$
%     \EndFor
%     \State $v\leftarrow \arg\min B$
%     \State $\mathvp\leftarrow \mathvp\backslash\{v\}$
% \EndWhile
% \State Return $\mathvp$
% \end{algorithmic}
% \end{small}
% \end{algorithm}


\myitem{Simple sorting algorithm.} We also study the performance of a simpler algorithm (Algorithm~\ref{alg:sorting}), which initially calculates for every \vp the resulting bias score if the \vp is removed from the set $\mathvp$, and then it removes (without further calculations) the $|\mathvp|-k$ vantage points that correspond to the lowest bias scores. The complexity of the algorithm is $O\left(|\mathvp|^{2}\right)$, which is significantly lower than the greedy. However, it is expected to perform worse than Algorithm~\ref{alg:subsampling-greedy}, since it does not take into account the combined effects of removing multiple \vps.  

% \begin{algorithm}
% \begin{small}
% \begin{algorithmic}[1]
% \caption{Subsampling - Sorting}\label{alg:sorting}
% \Statex {Input: $\mathcal{N}$ (population), $\mathvp$ (vantage points), $k$ (sample size)} 
% \For{$v\in\mathvp$}
%     \State $B_{v} \leftarrow calculate\_bias(\mathcal{N}, \mathvp\backslash\{v\})$
% \EndFor
% \While{$|\mathvp|>k$}
%     \State $v\leftarrow \arg\min B$
%     \State $\mathvp\leftarrow \mathvp\backslash\{v\}$
% \EndWhile
% \State Return $\mathvp$
% \end{algorithmic}
% \end{small}
% \end{algorithm}


% \begin{algorithm}
% % \begin{small}
% \begin{algorithmic}[1]
% \caption{Subsampling - Greedy}\label{alg:greedy}
% \Statex {Input: $\mathcal{N}$ (population), $\mathvp$ (monitors), $k$ (sample size)} 
% \While{$|\mathvp|>k$}
%     \State $\mathvp\leftarrow subsampling\_sorting(\mathcal{N},\mathvp,|\mathvp|-1)$
% \EndWhile
% \State Return $\mathvp$
% \end{algorithmic}
% % \end{small}
% \end{algorithm}


\subsection{Subsampling efficiency}\label{sec:subsampling-results}
Figure~\ref{fig:bias-vs-sample-size-greedy-all} shows the bias score (y-axis) for subsets of the \imps selected by the greedy Algorithm~\ref{alg:subsampling-greedy} (continuous lines) or the simple sorting Algorithm~\ref{alg:sorting} (dashed lines) for varying set sizes $k$ (x-axis). The bias score values at the rightmost part of the curves correspond to the bias score of the entire set of \vps $\mathvp$. As we move on the left of the x-axis, the subsampling algorithms remove \vps from $\mathvp$. In all cases, the subsampling with the greedy algorithm has a similar behavior: the bias score decreases as we remove \vps (i.e., moving to the left of the x-axis) to a minimum point, and then it increases again as the subset sizes become small. The minimum is achieved at samples sizes $k$ that are one order of magnitude less than the size of the entire \imp $|\mathvp|$ (note the log scale of the x-axis).

\myitem{RIPE RIS and RouteViews: the sweet spot of 50 peers.} RIPE RIS and RouteViews have a similar behavior, with sample sizes of around 50 \vps achieving the lowest bias score values of less than 0.04, which is \textit{four times lower than the bias score of the entire \vps sets}. Comparing the curves with this of random sampling in Fig.~\ref{fig:bias-vs-sample-size-total}, we see that for sample sizes $k<100$ \vps, the subsampling algorithm can select sets that have lower bias than what a random sample (of the same size) from the entire population of networks has.

\myitem{RIPE Atlas: almost zero bias with a few hundreds of probes.} In the case of RIPE Atlas the bias score is less than 0.01 (i.e., six times lower than the entire set of Atlas \vps) for subsets of a few hundreds of \vps ($84 \leq k \leq 976$). The minimum is achieved for around 300 \vps, and the greedy algorithm performs better than random sampling for samples smaller than $\sim$1,000 \vps. 

\myitem{Greedy vs. Sorting.} Finally, we compare the performance of the greedy algorithm (continuous lines) against the simple sorting algorithm (dashed lines). For large subset sizes ($k> 200$ for RIPE RIS and RouteViews, and $k>2000$ for Atlas) the performance of both algorithms is similar. However, as the subset sizes decrease, the sorting algorithm performs worse, since it does not take into account in its decisions the combined effect of removing more than one \vps.%; its decisions are based on the effect that the removal of a monitor would bring wrt. to the entire set of infrastructure.

And, while for RIPE RIS and RouteViews the minimum achieved bias score by the sorting algorithm (0.05 and 0.04, respectively) is not far from the corresponding of the greedy algorithm (25\%--30\% higher), in the case of RIPE Atlas the sorting algorithm achieves at best a 3 times higher bias score and for a much larger subset size $k$ (more than 1000 \vps). Nevertheless, the computation complexity of the sorting algorithm is much lower\footnote{In our experiments the greedy algorithm needed significantly more time, e.g., several minutes for RIPE RIS and RouteViews, and hours for RIPE Atlas.}. Hence, there is a trade-off between computational complexity and performance, and depending on the needs (e.g., real-timeness or resources) one can select which algorithm to use.


\textit{Remark:} The subsampling algorithms can be applied to any set $\mathvp$. For example, Fig.~\ref{fig:bias-vs-sample-size-greedy-Atlas-only} shows the results for a scenario where the algorithms received as input a random set of 300 RIPE Atlas \vps (``Atlas Rnd. 300''; purple lines). The greedy algorithm efficiently decreases the bias score from a value of 0.07 (for the entire random sample of 300 \vps)  to a value of 0.02 (achieved at the subset of 90 \vps). This is worse than applying the subsampling on the entire set of Atlas \vps (green lines), however, it comes at a much lower computational complexity.



\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=0.4\linewidth]{figures/fig_bias_vs_sampling_naive_and_greedy_ALL.png}\label{fig:bias-vs-sample-size-greedy-all}}
    \hspace{0.1\linewidth}
    \subfigure[]{\includegraphics[width=0.4\linewidth]{figures/fig_bias_vs_sampling_naive_and_greedy_only_Atlas.png}\label{fig:bias-vs-sample-size-greedy-Atlas-only}}
    \caption{Subsampling and bias: Bias score (y-axis) for subsets of infrastructure of different sizes (x-axis) as selected by the \textit{greedy} and the \textit{sorting} algorithms, for (a) RIPE Atlas, RIPE RIS, and RouteViews (RV), and (b) for the entire set and random subset of 300 monitors of RIPE Atlas.}
    \label{fig:}
\end{figure}

\subsection{Subsampling in the wild: a use case}\label{sec:cdn-use-case}

In this section we demonstrate through a use case how subsampling can improve measurement methodologies. 

\myitem{Use case: estimation of latency distribution.} We consider a measurement scenario where the goal is to estimate the distribution of the latency between a network (e.g., a content distribution network, CDN) and its client networks. A network may already have a custom measurement system to monitor the latency between all its customers. However, in some cases having a system like this may not be possible, and we may need to rely on \imps (e.g., ping measurements). For example, we may want to test a routing configuration that does not serve traffic, or evaluate the expected performance of a non-existing deployment~\cite{mcquistin2019taming}.

More specifically, let $\ell_{i}$ be the latency between the network and a client network $i$, and $L$ be the distribution of the latency values $\ell_{i}$ for all client networks $i\in\mathcal{N}$. Also, let us consider measurements from a subset $S$ of the infrastructure, $S\subseteq\mathvp$, and $L_{S}$ the distribution of the latency values for the networks $i\in S$. We want to investigate whether sets $S$ of lower bias results to a distribution $L_{S}$ that better approximates the ground-truth distribution $L$.\footnote{Note that our goal is simply to investigate the role of the set $S$ in the accuracy of a simple estimator $L_{S}$. Designing a fine-tuned methodology for accurately estimating the latency distribution from a set of measurements is out of the scope of this paper.}

\myitem{Experiment setup.} We conduct our experiment from a large production CDN with multiple points of presence and global coverage.
\begin{itemize}[leftmargin=*,nosep]
    \item \textit{Groundtruth latency data:} We collect client latency data (RTT) for all client ASes from the CDN monitoring infrastructure using TCP socket estimates, similar to~\cite{schlinker2019internet}. For each client AS, we collect multiple latency samples (from connections to different hosts in the same AS) and calculate the median\footnote{Considering other values (e.g., averages or minimum) did not affect our findings.} latency value $\ell_{i}$ per AS $i$. 
    \item \textit{RIPE Atlas measurements:} We conduct ping measurements from all RIPE Atlas probes to %an endpoint served by 
    the same global CDN infrastructure as measured in the previous step, and collect the RTT values. For ASes hosting more than one probes, we calculate the median latency, which we denote as $\ell_{i}^{'}$ for an AS $i$. 
\end{itemize}
We calculate the latency distribution of the ground-truth data $L$ from the CDN measurements over all ASes, i.e., $\{\ell_{i}: \forall i\in\mathcal{N}\}$. We want to investigate how accurately we can estimate $L$ with the RIPE Atlas platform. Hence, we consider the following subsets $S$ of the RIPE Atlas platform:
\begin{itemize}[leftmargin=*,nosep]
    \item \textit{Atlas All:} $S=\mathvp$, i.e., all ASes that host at least one RIPE Atlas probe.
    \item \textit{Greedy (k=300):} The set $S$ selected by Algorithm~\ref{alg:subsampling-greedy} for size set $k=300$, i.e., the subset with the minimum bias score (see~\secref{sec:subsampling-results} and Fig.~\ref{fig:bias-vs-sample-size-greedy-all}).
    % \item \textit{Atlas greedy 1000:} The set $S$ selected by the subsampling Algorithm~\ref{alg:subsampling-greedy} for size set $k=1000$. We consider this set as a comparison, since it has slightly higher bias score than \textit{Atlas greedy 300} but significantly more monitors.
    \item \textit{Random (k=300):} A set $S$ consisting of a random sample of 300 Atlas probes. For statistical significance, we consider 10 different sets.
\end{itemize}
For each set $S$, we calculate two latency distributions: 
The \textit{actual measurement distribution} $L_{S}^{'}$, which consists of the RTT values from the RIPE Atlas measurements $\ell_{i}^{'}$, $i\in S$, and the \textit{simulated measurement distribution}, $L_{S}$, which consists of the values of the CDN measurements $\ell_{i}$, $i\in S$. The reason for this additional consideration is to isolate any noise due to methodological differences between RIPE Atlas and CDN measurements per AS, i.e., differences between $\ell_{i}$ and $\ell_{i}^{'}$.




\begin{figure}
    \centering
    \subfigure[RIPE Atlas measurements]{\includegraphics[width=0.4\linewidth]{figures/fig_cdn_errors_atlas.png}\label{fig:cdn-error-atlas}}
    \hspace{0.1\linewidth}
    \subfigure[CDN measurements]{\includegraphics[width=0.4\linewidth]{figures/fig_cdn_errors_simulated.png}\label{fig:cdn-error-simulated}}
    \caption{Relative error between the groundtruth distribution $L$ and the measured distribution of (a) actual RIPE Atlas measurements $L_{S}^{'}$, and (b) simulated measurements $L_{S}$. The curve for the random sets corresponds to the average over 10 random sets (black line) with confidence intervals (errorbars), and the grey area to the max/mix~values.}
    \label{fig:cdn-error}
\end{figure}




\myitem{Results.} Figure~\ref{fig:cdn-error} presents the relative error (y-axis) between the measured latency distribution $L_{S}^{'}$ and the groundtruth distribution $L$ for all percentiles (x-axis). For example, if the $30^{th}$ percentile of $L_{S}$ is $t$ sec. ($L_{S}(30) = t$) and the corresponding percentile for $L$ is $L(30)=0.8\cdot t$ sec., then the relative error is $\frac{|L_{S}(30)-L(30)|}{L(30)} = \frac{|t-0.8\cdot t|}{0.8\cdot t}=0.25$. 

We can see that the relative error for the subset selected by the greedy algorithm (blue lines) is lower than the relative error of the entire set of Atlas \vps (orange lines) and the average relative error of the randomly selected sets (black lines) in the majority of the percentiles. For low percentiles (e.g., less than 20\%) the subsets selected by the greedy show a higher relative error, however, due to the fact that these percentiles correspond to latency values of a few milliseconds, small differences in the measured latencies lead to high relative errors (see the higher variability of the random results indicated by the gray area). Taking into account the accuracy over the entire distribution (i.e., average accuracy over all the percentiles), the subsampling achieves almost one third lower errors than using the entire set of Atlas probes or random sets of them (see Table~\ref{table:average-error-cdn}).

The same trends holds both for the RIPE Atlas measurements (Fig.~\ref{fig:cdn-error-atlas}) and the CDN measurements (Fig.~\ref{fig:cdn-error-simulated}); in the latter, the errors are lower due to the isolation of the "noise" from the different measurement methodologies. 

These results indicate that subsampling for sets of lower bias can improve measurement methodologies. Further refinements in the subsampling per use case, e.g., identifying the bias dimensions that relate to latency measurements and taking only them into account, could lead to higher accuracy (see~\secref{sec:conclusion}). 


\begin{table}
    \centering
    \caption{Average relative error (over all percentiles) in latency measurements.}
    % \begin{small}
    % \begin{tabular}{l|cc}
    % Selected set & RIPE Atlas msmt. & CDN msmt.\\
    % \hline
    %  Greedy (k=300) &  26\% & 12\%\\
    %  Atlas All      &  31\% & 18\%  \\
    %  Random (k=300) &  32\% & 18\%
    %  \end{tabular}
    % \end{small}
    \begin{small}
    \begin{tabular}{l||c|c|c}
    Measurements & Greedy (k=300) & Atlas All & Random (k=300) \\
    \hline
     RIPE Atlas &  26\% & 31\% & 32\%\\
     CDN      &  12\% & 18\%  & 18\%
     \end{tabular}
    \end{small}
    \label{table:average-error-cdn}
\end{table}


\myitem{Summary of main takeaways:} \one We extended our framework with subsampling methods that allow users to choose low-bias subsets of the \vps of an \imp; \two While choosing sets of \textasciitilde50 vantage point from RIPE RIS and \rv can decrease the bias 3.25-fold, greedily choosing a set of \textasciitilde300 RIPE Atlas vantage points can almost entirely eliminate bias; \three A first in-the-wild test of our subsampling methods showed that its selection of RIPE Atlas probes can improve the prediction of the global latency distribution for a large anycast CDN. 




